Self-Tuning: Instructing LLMs to Effectively Acquire New Knowledge through Self-Teaching

Large language models (LLMs) often struggle to provide up-to-date information due to their one-time training and the constantly evolving nature of the world. To keep LLMs current, existing approaches typically involve continued pre-training on new documents. However, they frequently face difficulties in extracting stored knowledge. Motivated by the remarkable success of the Feynman Technique in efficient human learning, we introduce Self-Tuning, a learning framework aimed at improving an LLM's ability to effectively acquire new knowledge from unseen raw documents through self-teaching. Specifically, we develop a Self-Teaching strategy that augments the documents with a set of knowledge-intensive tasks created in a self-supervised manner, focusing on three crucial aspects: memorization, comprehension, and self-reflection. Additionally, we introduce three Wiki-Newpages-2023-QA datasets to facilitate an in-depth analysis of an LLM's knowledge acquisition ability concerning memorization, extraction, and reasoning. Extensive experimental results on various models, e.g., Llama2-7B reveal that Self-Tuning consistently exhibits superior performance across all knowledge acquisition tasks and excels in preserving previous knowledge.

==> sections/ethics.tex <==
Throughout our research, we have consistently adhered to ethical guidelines to uphold privacy, fairness, and the well-being of all individuals and groups involved. All benchmark datasets utilized in this study are used solely for research purposes and do not contain any personally identifiable information, thereby safeguarding privacy. During the QA data collection process for Wiki-Newpages-2023-QA, WikiBio-2024, and WebNews-2023 using GPT-4, we meticulously crafted prompts to eliminate any language that might discriminate against specific individuals or groups. These measures were implemented to minimize potential negative effects on users' well-being. Examples of these carefully designed prompts can be found in Table~\ref{tab:wikiqa_gen_prompt}, Table~\ref{tab:wikiqa_nli_prompt}, and Table~\ref{tab:wikiqa_type_prompt}. To further ensure the quality of the newly collected datasets, the authors manually reviewed them following the guidelines in \citet{bai2022constitutional}. These datasets were confirmed to be of high quality, free from offensive content, false information, and any personally identifiable information~\cite{radharapu-etal-2023-aart, zhou2023rethinking}. Future research efforts could explore the OpenAI moderation API\footnote{\url{https://platform.openai.com/docs/guides/moderation/overview}} to systematically filter out inappropriate system responses. Additionally, GPT-4 is solely used to convert document knowledge into QA pairs—without introducing any additional information—and can be replaced by any other model. 

% Our study is committed to advancing knowledge while maintaining strong ethical principles, ensuring privacy, fairness, and the well-being of all individuals and groups involved.

==> sections/experiments/results_varying_models_corpus.tex <==
% wiki-bio2024 from 2024 june-sep, test set, 827 qa pairs, 146 test texts.

% webnews data, training set qa 5032, 1500 texts.


% test set, qa 675, test texts 155


% We download a news
% dataset using the mediastack API 1
% , a REST API interface delivering worldwide news data. The news
% data source comprises various English-language
% websites covering a range of news categories: entertainment, business, sports, technology, health,
% and science. To mimic real-world RAG scenarios,
% where the knowledge base data, such as an enterprise’s internal data, may differ from the LLMs’
% training data, we select news articles published
% from September 26, 2023, to December 26, 2023.
% This timeframe extends beyond the knowledge cutoff of some widely-used LLMs, including ChatGPT and LLaMA, as of the time of writing. \footnote{\url{https://mediastack.com/}}

% Step 2: Evidence Extraction. For each article, we
% extract factual or opinion sentences using a trained
% language model 2
% . These factual sentences are later
% used as evidence for answering multi-hop queries.
% We retain only those news articles containing evidence that may have overlapping keywords with
% other news articles

% Step 3: Claim, Bridge-Entity, Bridge-Topic Generation. Our goal is to use GPT-4 to automatically
% generate high-quality multi-hop queries using the
% evidence set. However, the raw evidence obtained
% from Step 2 is not ideal for query generation due
% to inconsistency in linguistic structure. For example, some pieces of evidence use pronouns to refer
% to subjects and lack the actual entity in the text.
% To address this, we employ GPT-4 to paraphrase
% the evidence, which we refer to as claims, given
% the original evidence and its context. To ensure
% consistency between the generated claim and the
% evidence, we further perform fact-checking using
% the UniEval (Zhong et al., 2022) framework to verify the alignment between the evidence and claim.
% Appendix A presents the prompt used for GPT-4
% for claim generation.

==> sections/floats/table/table_bio_test_instruction.tex <==
\begin{table*}[!t]
\setlength\tabcolsep{1.5pt}
  \centering
  \begin{threeparttable}
  \fontsize{9}{10}
  \selectfont
    \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{4}{*}{\textbf{Method}}&
    \multicolumn{7}{c}{\textbf{Wiki-Newpages-2023-10-Bio (Acquisition)}} 
     &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & \textbf{Memorization}
      &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reasoning} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{Acc.}$\cr
    % \midrule
    % \multicolumn{11}{c}{\textbf{\textit{\llamaa{}}}}\cr
    \midrule
        \multicolumn{11}{c}{\textbf{\textit{\llamaa{}}}}\cr
    \midrule
    Closed-book &8.41&4.68&2.87&14.63&16.98&15.07 &7.96& 16.05&24.67&53.40\\
    \hdashline
    \noalign{\vskip 0.07cm} % Adds a small vertical space
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Con. Pre-training & 7.28&6.33&3.62&15.96&18.72&16.11 &15.09 & \textcolor{red}{16.00}&\textcolor{red}{24.11}&53.40\\
    \selfpt{}$^{-}$& 1.16& 36.95& \textbf{31.52} & 49.01& 50.24 & 48.82 &\textbf{51.58}& \textbf{16.56} & \textbf{26.09} & \textbf{67.73}\\
    \selfpt{} & \textbf{1.11}& \textbf{37.25}& \textbf{31.52} & \textbf{50.83}& \textbf{52.62} & \textbf{50.61} &44.31& 16.45 & 25.67 & 66.01\\
    \midrule
     \multicolumn{11}{c}{\textbf{\textit{\llamaathirteen{}}}}\cr
     \midrule
     Closed-book &8.27& 6.33 & 4.68 & 17.45 & 19.37 & 17.58 & 3.57 & 19.84 & 28.71 & 66.34\\
         \hdashline
    \noalign{\vskip 0.07cm} % Adds a small vertical space
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Con. Pre-training &  6.35 & \textcolor{red}{4.98} & \textcolor{red}{3.77} & \textcolor{red}{17.12} & \textcolor{red}{18.95} & \textcolor{red}{17.04} & 5.49 & \textbf{21.25} & 30.35&66.34 \\
     \selfpt{}$^{-}$& 1.11& 40.42& 36.50 & 53.77& 55.32 & 53.35 &53.09& 19.73 & 30.80& 71.74\\
    \selfpt{} & \textbf{1.09} & \textbf{44.19} & \textbf{39.37} & \textbf{58.31} & \textbf{60.47} & \textbf{57.90} & \textbf{54.18} & 20.69 & \textbf{31.62} & \textbf{71.50} \\
    \bottomrule  
    \end{tabular}
  \end{threeparttable}
    \caption{Ablation study on including summarization and ``teaching'' tasks during training on test documents. Results that fall short of closed-book performance without knowledge injection are highlighted in \textcolor{red}{red}.}
  \label{tab:ablation-test-instruct-bio-domain}
  \vspace{-1mm}
\end{table*}

==> sections/floats/table/table_cross_domain.tex <==
% \begin{table}[!t]
% \setlength\tabcolsep{1pt}
%   \centering
%   \begin{threeparttable}
%   \fontsize{9}{9}
%   \selectfont
%     \begin{tabular}{lcccccccccc}
%     \toprule
%     \multirow{2}{*}{Method}&
%     \multicolumn{6}{c}{\textbf{Wiki-2023-(9)10-Film (Acquisition)}}\cr\cmidrule(lr){2-7}
%      &\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$&$\mathtt{PPL}$ ($\downarrow$) \cr
%     \midrule
%     \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
%     Open-book w/ doc &57.38 & 34.45&68.64&78.92&66.31&-\\
%     Closed-book &3.35&1.88&11.27&12.97&11.49&8.30\\
%     % \midrule
%     % \hdashline
%     \midrule
%    % \noalign{\vskip 0.07cm} % Adds a small vertical space
%    % \multicolumn{10}{l}{\cellcolor{lightgray!25}{+ \ski{}}}\cr 
%    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
%     Conti. Pre-training &3.25&2.30&11.83&14.30&11.98&4.96\\
%     + via Read. Comp. &2.72&1.68&9.81&14.94&10.02&9.21\\
%     + w/ Self-Exam. &12.77&10.47&24.71&31.06&24.66&0.71\\
%     \hdashline
%     \noalign{\vskip 0.07cm} % Adds a small vertical space
%     Standard Ins.-Tun. & 5.23& 3.77&16.15&17.45&16.45&1.52 \\
%     Mixed Training & 11.41 & 9.63 & 23.61 & 24.48 &23.67 & 0.76 \\
%      PIT & 6.39 & 4.50 & 16.97&18.92&17.10&1.52 \\
%      Self-Exam. Pre-Tun. & 24.50 & 19.06 & 37.40 & 38.27 & 37.15 & 0.95\\

%     \bottomrule  
%     \end{tabular}
%   \end{threeparttable}
  
%   \caption{Five-shot evaluation results on knowledge acquisition in the cross-domain scenario.}
%   \label{tab:film-domain}
%   \vspace{-1mm}
% \end{table}

\begin{table*}[!t]
\setlength\tabcolsep{1.5pt}
  \centering
  \begin{threeparttable}
  \fontsize{9}{9}
  \selectfont
    \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{4}{*}{\textbf{Method}}&
    \multicolumn{7}{c}{\textbf{Wiki-Newpages-2023-(9)10-Film (Acquisition)}} 
     &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & \textbf{Memorization}
      &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reason.} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{Acc.}$\cr
        \midrule
    \multicolumn{11}{c}{\textbf{\textit{\llamaa{}}}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ film doc &8.30&57.38 & 34.45&68.64&78.92&66.31&7.35&-&-&-\\
    Closed-book &8.30&3.35&1.88&11.27&12.97&11.49&7.35&16.05&24.67&53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Cont. Pre-training &5.52 &3.46&2.30&11.83&14.30&11.98&12.04&16.79& 25.35 & 56.02\\
    % \hdashline
    % \noalign{\vskip 0.07cm} % Adds a small vertical space
    Standard Ins.-tuning &2.83& 5.23 & 3.77& 16.15& 17.45& 16.45& 51.69& \textcolor{red}{14.41}& 25.54 & \textcolor{red}{49.80} \\ 

     Mixed Training &1.47&  11.41& 9.63 & 23.61&24.48 & 23.67 & \textbf{59.99}&\textbf{17.35}&\textbf{27.79} &58.56\\
     
     PIT&1.52& 6.39 & 2.67& 16.97 & 18.92& 17.10 &3.03&\textcolor{red}{13.06} & \textcolor{red}{23.42} & 54.38 \\

     \selfpt{} & \textbf{1.10} & \textbf{22.51}& \textbf{16.44} & \textbf{35.58}& \textbf{36.60} & \textbf{35.43} & 44.92& 16.77& 26.44 & \textbf{66.34}\\ 
     
     \selfpt{}$^{++}$ & \textbf{1.10}& \textbf{23.66}& \textbf{17.49} & \textbf{37.16}& \textbf{38.56} & \textbf{37.03} &  46.79 & \textcolor{red}{16.00} & \textcolor{red}{26.03} & \textbf{66.58}\\
    \bottomrule  
    \end{tabular}
  \end{threeparttable}
  
  \caption{Five-shot evaluation results on knowledge acquisition and retention in the cross-domain scenario, where the training data is Wiki-Bio, the testing data is Wiki-Film. Results that are inferior to closed-book performance without knowledge injection are indicated in \textcolor{red}{red}.}
  \label{tab:film-domain}
  % \vspace{-1mm}
\end{table*}



==> sections/floats/table/table_hard_bio_complete.tex <==
% \begin{table*}[!t]
% \setlength\tabcolsep{2pt}
%   \centering
%   \begin{threeparttable}
%   \fontsize{9}{10}
%   \selectfont
%     \begin{tabular}{lcccccccccccc}
%     \toprule
%     \multirow{4}{*}{\textbf{Method}}&
%     \multicolumn{7}{c}{\textbf{Wiki-Newpages-2023-10-Biography (Acquisition)}} 
%      &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
%      & \textbf{Memorization}
%       &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reason.} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
%      & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{EM}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{EM}$\cr
%     \midrule
%     \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
%     Open-book w/ test doc &28.19&55.20& 31.83&64.48&75.55&62.10& 7.96&-&-&-\\
%     Closed-book &28.19&4.68&2.87&14.63&16.98&15.07 &7.96& 16.05&24.67&53.40\\
%     \midrule
%    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
%     Cont. Pre-training & 9.48&6.33&3.62&15.96&18.72&16.11 &15.09 & \textcolor{red}{16.00}&\textcolor{red}{24.11}&53.40\\
    
%     Standard Ins.-tuning & 2.44& 6.94 & 5.13& 19.15& 19.05& 19.48&39.09& \textcolor{red}{15.72}& \textcolor{red}{23.67} & \textcolor{red}{51.84}  \\ 
    
%      Mixed Training &1.16&  25.34& 21.57 & 38.56&39.76 & 38.64 &27.71&\textbf{19.50}&\textbf{28.05} &58.97 \\ 
     
%      PIT & 1.12& 14.03 & 11.61& 27.15 & 28.86& 27.11 &11.93& \textcolor{red}{15.72}& 26.31 & 57.58\\
     
%     \selfpt{} & \textbf{1.10}& \textbf{37.25}& \textbf{31.52} & \textbf{50.83}& \textbf{52.62} & \textbf{50.61} &\textbf{44.31}& 16.45 & 25.67 & \textbf{66.01}\\
    
%      \selfpt{}$^{++}$ & \textbf{1.02} & \textbf{41.33}& \textbf{36.65} & \textbf{53.99}& \textbf{55.57} & \textbf{53.80}  & \textbf{47.87} & 16.68 & 26.11 & \textbf{66.75}\\
%     \hdashline
%     \noalign{\vskip 0.07cm} % Adds a small vertical space
%     \selfpt{} via Read. & 1.36& 19.46 & 16.74& 34.12 & 35.17& 34.04 &40.74& 19.56& 27.95 & 65.02\\
      
%     \selfpt{} w/ Pre-con. & 1.11& 29.86& 25.94 & 43.46& 44.96 & 43.31 &46.91 & 16.28 & 24.80 & 65.11\\
%     \bottomrule  
%     \end{tabular}
%   \end{threeparttable}
%   \caption{Evaluation results on knowledge acquisition in the single-domain scenario.}
%   \label{tab:hard-bio-domain}
%   \vspace{-1mm}
% \end{table*}


\begin{table*}[!t]
\setlength\tabcolsep{2.5pt}
  \centering
  \begin{threeparttable}
  \fontsize{9}{10}
  \selectfont
    \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{4}{*}{\textbf{Method}}&
    \multicolumn{7}{c}{\textbf{Wiki-Newpages-2023-QA (Acquisition)}} 
     &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & \textbf{Memorization}
      &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reason.} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{Acc.}$\cr
    \midrule
    \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-10-Bio (Single-Domain Scenario)}}\cr
    % \multicolumn{11}{c}{\textbf{\textit{\llamaa{}}}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ test doc &8.41&55.20& 31.83&64.48&75.55&62.10& 7.96&-&-&-\\
    Closed-book &8.41&4.68&2.87&14.63&16.98&15.07 &7.96& 16.05&24.67&53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Cont. Pre-training & 7.28&6.33&3.62&15.96&18.72&16.11 &15.09 & \textcolor{red}{16.00}&\textcolor{red}{24.11}&53.40\\
    
    Standard Ins.-tuning & 6.83& 6.94 & 5.13& 19.15& 19.05& 19.48&39.09& \textcolor{red}{15.72}& \textcolor{red}{23.67} & \textcolor{red}{51.84}  \\ 
    
     PIT & 2.08& 14.03 & 11.61& 27.15 & 28.86& 27.11 &11.93& \textcolor{red}{15.72}& \textbf{26.31} & 57.58\\
    \selfpt{} & \textbf{1.11}& \textbf{37.25}& \textbf{31.52} & \textbf{50.83}& \textbf{52.62} & \textbf{50.61} &\textbf{44.31}& \textbf{16.45} & 25.67 & \textbf{66.01}\\

    \midrule
        \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-10-Multi (Multi-Domain Scenario)}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ test doc & 7.84&48.93&26.63&60.37&71.71&58.54&6.33&-&-&-\\
    Closed-book & 7.84&4.53&2.73&16.19&18.63&16.38&6.33&16.05&24.67 & 53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Cont. Pre-training & 3.32&5.86&3.40&18.04&20.59&18.42&14.51&\textbf{17.02}&25.05&53.56\\
    
    Standard Ins.-tuning & 2.73& 8.66 & 5.73& 24.94& 25.64& 25.31 & 34.91& \textcolor{red}{15.60}& 26.26 & \textcolor{red}{52.74} \\ 
    
     % Mixed Training & 1.47 &  16.91& 12.25 & 34.48&35.20 & 34.41 &29.44&\textbf{17.75}&\textbf{28.68} &59.38\\ 
     
     PIT & 1.96& 14.31 & 8.72& 30.26 & 33.97& 30.22 &10.69&\textcolor{red}{15.55} & \textbf{27.02} & 55.12 \\ 
     
      \selfpt{} & \textbf{1.13} & \textbf{22.30}& \textbf{16.51} & \textbf{39.94}& \textbf{41.02} & \textbf{39.89}  & \textbf{50.65}& 16.34 & 25.85 & \textbf{69.29}\\ 
      
       % \selfpt{}$^{++}$ & \textbf{1.09} & \textbf{24.70}& \textbf{17.78} & \textbf{42.95}& \textbf{44.31} & \textbf{42.71} & \textbf{52.61}& \textcolor{red}{14.47} & 25.25 & 66.83\\ 

        \midrule
    \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-(9)10-Film (Cross-Domain Scenario)}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ film doc &8.30&57.38 & 34.45&68.64&78.92&66.31&7.35&-&-&-\\
    Closed-book &8.30&3.35&1.88&11.27&12.97&11.49&7.35&16.05&24.67&53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Cont. Pre-training &5.52 &3.46&2.30&11.83&14.30&11.98&12.04&\textbf{16.79}& 25.35 & 56.02\\
    % \hdashline
    % \noalign{\vskip 0.07cm} % Adds a small vertical space
    Standard Ins.-tuning &2.83& 5.23 & 3.77& 16.15& 17.45& 16.45& \textbf{51.69}& \textcolor{red}{14.41}& 25.54 & \textcolor{red}{49.80} \\ 

     % Mixed Training &1.47&  11.41& 9.63 & 23.61&24.48 & 23.67 & \textbf{59.99}&\textbf{17.35}&\textbf{27.79} &58.56\\
     
     PIT&1.52& 6.39 & 4.50& 16.97 & 18.92& 17.10 &3.03&\textcolor{red}{13.06} & \textcolor{red}{23.42} & 54.38 \\

     \selfpt{} & \textbf{1.10} & \textbf{22.51}& \textbf{16.44} & \textbf{35.58}& \textbf{36.60} & \textbf{35.43} & 44.92& 16.77& \textbf{26.44} & \textbf{66.34}\\ 
     % \selfpt{}$^{++}$ &\textbf{1.08} & \textbf{44.49}& \textbf{39.82} & \textbf{58.44}& \textbf{60.58} & \textbf{58.00}  & 53.91 & 20.46 & \textbf{32.01} & \textbf{72.48}\\
    \bottomrule  
    \end{tabular}
  \end{threeparttable}
  \caption{Five-shot evaluation results on \llamaa{} for knowledge acquisition and retention in three scenarios: single-domain (top), multi-domain (middle), and cross-domain (bottom). Results that fall below the baseline performance are highlighted in \textcolor{red}{red}.}
  \label{tab:hard-bio-domain}
  % \vspace{-3.5mm}
\end{table*}

%In the cross-domain scenario, the training data comes from Wiki-Bio, while the testing data is from Wiki-Film.

==> sections/floats/table/table_hard_multi_task.tex <==
\begin{table*}[!t]
\setlength\tabcolsep{2pt}
  \centering
  \begin{threeparttable}
  \fontsize{9}{10}
  \selectfont
    \begin{tabular}{lccccccccccc}
    \toprule
    \multirow{4}{*}{\textbf{Method}}&
    \multicolumn{7}{c}{\textbf{Acquisition}} 
     &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & \textbf{Memorization}
      &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reason.} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{Acc.}$\cr
    \midrule
    \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-10-Multi (Multi-Domain Scenario)}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ test doc & 7.84&48.93&26.63&60.37&71.71&58.54&6.33&-&-&-\\
    Closed-book & 7.84&4.53&2.73&16.19&18.63&16.38&6.33&16.05&24.67 & 53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Cont. Pre-training & 3.32&5.86&3.40&18.04&20.59&18.42&14.51&\textbf{17.02}&25.05&53.56\\
    
    Standard Ins.-tuning & 2.73& 8.66 & 5.73& 24.94& 25.64& 25.31 & 34.91& \textcolor{red}{15.60}& 26.26 & \textcolor{red}{52.74} \\ 
    
     % Mixed Training & 1.47 &  16.91& 12.25 & 34.48&35.20 & 34.41 &29.44&\textbf{17.75}&\textbf{28.68} &59.38\\ 
     
     PIT & 1.96& 14.31 & 8.72& 30.26 & 33.97& 30.22 &10.69&\textcolor{red}{15.55} & \textbf{27.02} & 55.12 \\ 
     
      \selfpt{} & \textbf{1.13} & \textbf{22.30}& \textbf{16.51} & \textbf{39.94}& \textbf{41.02} & \textbf{39.89}  & \textbf{50.65}& 16.34 & 25.85 & \textbf{69.29}\\ 
      
       % \selfpt{}$^{++}$ & \textbf{1.09} & \textbf{24.70}& \textbf{17.78} & \textbf{42.95}& \textbf{44.31} & \textbf{42.71} & \textbf{52.61}& \textcolor{red}{14.47} & 25.25 & 66.83\\ 

        \midrule
    \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-(9)10-Film (Cross-Domain Scenario)}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ film doc &8.30&57.38 & 34.45&68.64&78.92&66.31&7.35&-&-&-\\
    Closed-book &8.30&3.35&1.88&11.27&12.97&11.49&7.35&16.05&24.67&53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Cont. Pre-training &5.52 &3.46&2.30&11.83&14.30&11.98&12.04&\textbf{16.79}& 25.35 & 56.02\\
    % \hdashline
    % \noalign{\vskip 0.07cm} % Adds a small vertical space
    Standard Ins.-tuning &2.83& 5.23 & 3.77& 16.15& 17.45& 16.45& \textbf{51.69}& \textcolor{red}{14.41}& 25.54 & \textcolor{red}{49.80} \\ 

     % Mixed Training &1.47&  11.41& 9.63 & 23.61&24.48 & 23.67 & \textbf{59.99}&\textbf{17.35}&\textbf{27.79} &58.56\\
     
     PIT&1.52& 6.39 & 2.67& 16.97 & 18.92& 17.10 &3.03&\textcolor{red}{13.06} & \textcolor{red}{23.42} & 54.38 \\

     \selfpt{} & \textbf{1.10} & \textbf{22.51}& \textbf{16.44} & \textbf{35.58}& \textbf{36.60} & \textbf{35.43} & 44.92& 16.77& \textbf{26.44} & \textbf{66.34}\\ 
     
     % \selfpt{}$^{++}$ & \textbf{1.10}& \textbf{23.66}& \textbf{17.49} & \textbf{37.16}& \textbf{38.56} & \textbf{37.03} &  46.79 & \textcolor{red}{16.00} & 26.03 & \textbf{66.58}\\
    \bottomrule  
    \end{tabular}
  \end{threeparttable}
  
  \caption{Five-shot evaluation results on knowledge acquisition and retention in the multi-domain (upper) and cross-domain scenarios (lower). In the cross-domain scenario, the training data comes from Wiki-Bio, while the testing data is from Wiki-Film. Results that fall below the baseline performance are highlighted in \textcolor{red}{red}.}
  \label{tab:hard-multi-domain_complete}
  \vspace{-1mm}
\end{table*}

% \begin{table*}[!t]
% \setlength\tabcolsep{1.5pt}
%   \centering
%   \begin{threeparttable}
%   \fontsize{9}{9}
%   \selectfont
%     \begin{tabular}{lcccccccccc}
%     \toprule
%     \multirow{4}{*}{\textbf{Method}}&
%     \multicolumn{7}{c}{\textbf{Wiki-Newpages-2023-(9)10-Film (Acquisition)}} 
%      &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
%      & \textbf{Memorization}
%       &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reason.} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
%      & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{EM}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{EM}$\cr
%         \midrule
%     \multicolumn{11}{c}{\textbf{\textit{\llamaa{}}}}\cr
%     \midrule
%     \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
%     Open-book w/ film doc &8.30&57.38 & 34.45&68.64&78.92&66.31&7.35&-&-&-\\
%     Closed-book &8.30&3.35&1.88&11.27&12.97&11.49&7.35&16.05&24.67&53.40\\
%     \midrule
%    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
%     Cont. Pre-training &5.52 &3.46&2.30&11.83&14.30&11.98&12.04&16.79& 25.35 & 56.02\\
%     % \hdashline
%     % \noalign{\vskip 0.07cm} % Adds a small vertical space
%     Standard Ins.-tuning &2.83& 5.23 & 3.77& 16.15& 17.45& 16.45& 51.69& \textcolor{red}{14.41}& 25.54 & \textcolor{red}{49.80} \\ 

%      Mixed Training &1.47&  11.41& 9.63 & 23.61&24.48 & 23.67 & \textbf{59.99}&\textbf{17.35}&\textbf{27.79} &58.56\\
     
%      PIT&1.52& 6.39 & 2.67& 16.97 & 18.92& 17.10 &3.03&\textcolor{red}{13.06} & \textcolor{red}{23.42} & 54.38 \\

%      \selfpt{} & \textbf{1.10} & \textbf{22.51}& \textbf{16.44} & \textbf{35.58}& \textbf{36.60} & \textbf{35.43} & 44.92& 16.77& 26.44 & \textbf{66.34}\\ 
     
%      \selfpt{}$^{++}$ & \textbf{1.10}& \textbf{23.66}& \textbf{17.49} & \textbf{37.16}& \textbf{38.56} & \textbf{37.03} &  46.79 & \textcolor{red}{16.00} & \textcolor{red}{26.03} & \textbf{66.58}\\
%     \bottomrule  
%     \end{tabular}
%   \end{threeparttable}
  
%   \caption{ Results that are inferior to closed-book performance without knowledge injection are indicated in \textcolor{red}{red}.}
%   \label{tab:film-domain}
%   \vspace{-1mm}
% \end{table*}



==> sections/floats/table/table_short_main_results.tex <==
% \begin{table*}[!t]
% \setlength\tabcolsep{2pt}
%   \centering
%   \begin{threeparttable}
%   \fontsize{9}{10}
%   \selectfont
%     \begin{tabular}{lcccccccccccc}
%     \toprule
%     \multirow{4}{*}{\textbf{Method}}&
%     \multicolumn{7}{c}{\textbf{Wiki-Newpages-2023-10-Biography (Acquisition)}} 
%      &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
%      & \textbf{Memorization}
%       &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reason.} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
%      & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{EM}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{EM}$\cr
%     \midrule
%     \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
%     Open-book w/ test doc &28.19&55.20& 31.83&64.48&75.55&62.10& 7.96&-&-&-\\
%     Closed-book &28.19&4.68&2.87&14.63&16.98&15.07 &7.96& 16.05&24.67&53.40\\
%     \midrule
%    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
%     Cont. Pre-training & 9.48&6.33&3.62&15.96&18.72&16.11 &15.09 & \textcolor{red}{16.00}&\textcolor{red}{24.11}&53.40\\
    
%     Standard Ins.-tuning & 2.44& 6.94 & 5.13& 19.15& 19.05& 19.48&39.09& \textcolor{red}{15.72}& \textcolor{red}{23.67} & \textcolor{red}{51.84}  \\ 
    
%      Mixed Training &1.16&  25.34& 21.57 & 38.56&39.76 & 38.64 &27.71&\textbf{19.50}&\textbf{28.05} &58.97 \\ 
     
%      PIT & 1.12& 14.03 & 11.61& 27.15 & 28.86& 27.11 &11.93& \textcolor{red}{15.72}& 26.31 & 57.58\\
     
%     \selfpt{} & \textbf{1.10}& \textbf{37.25}& \textbf{31.52} & \textbf{50.83}& \textbf{52.62} & \textbf{50.61} &\textbf{44.31}& 16.45 & 25.67 & \textbf{66.01}\\
    
%      \selfpt{}$^{++}$ & \textbf{1.02} & \textbf{41.33}& \textbf{36.65} & \textbf{53.99}& \textbf{55.57} & \textbf{53.80}  & \textbf{47.87} & 16.68 & 26.11 & \textbf{66.75}\\
%     \hdashline
%     \noalign{\vskip 0.07cm} % Adds a small vertical space
%     \selfpt{} via Read. & 1.36& 19.46 & 16.74& 34.12 & 35.17& 34.04 &40.74& 19.56& 27.95 & 65.02\\
      
%     \selfpt{} w/ Pre-con. & 1.11& 29.86& 25.94 & 43.46& 44.96 & 43.31 &46.91 & 16.28 & 24.80 & 65.11\\
%     \bottomrule  
%     \end{tabular}
%   \end{threeparttable}
%   \caption{Evaluation results on knowledge acquisition in the single-domain scenario.}
%   \label{tab:hard-bio-domain}
%   \vspace{-1mm}
% \end{table*}


\begin{table*}[!t]
\setlength\tabcolsep{2.5pt}
  \centering
  \begin{threeparttable}
  \fontsize{9}{10}
  \selectfont
    \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{4}{*}{\textbf{Method}}&
    \multicolumn{7}{c}{\textbf{Wiki-Newpages-2023-QA (Acquisition)}} 
     &\multicolumn{2}{c}{\textbf{NQ (Reten.)}} &\textbf{CSQA (Reten.)}\cr\cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & \textbf{Memorization}
      &\multicolumn{5}{c}{\textbf{Extraction}}&\textbf{Reason.} &\multicolumn{2}{c}{\textbf{Extraction}}&\textbf{Reasoning} \cr\cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11}
     & $\mathtt{PPL}$ ($\downarrow$)&\%  $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$&\%  $\mathtt{Rec.}$&\%  $\mathtt{Rouge}$ &\% $\mathtt{Acc.}$ &\%  $\mathtt{EM}$ &\%  $\mathtt{F1}$ &\%  $\mathtt{Acc.}$\cr
    \midrule
    \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-10-Bio (Single-Domain Scenario)}}\cr
    % \multicolumn{11}{c}{\textbf{\textit{\llamaa{}}}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ test doc &8.41&55.20& 31.83&64.48&75.55&62.10& 7.96&-&-&-\\
    Closed-book &8.41&4.68&2.87&14.63&16.98&15.07 &7.96& 16.05&24.67&53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Con. Pre-training & 7.28&6.33&3.62&15.96&18.72&16.11 &15.09 & \textcolor{red}{16.00}&\textcolor{red}{24.11}&53.40\\
    
    Standard Ins.-tuning & 6.83& 6.94 & 5.13& 19.15& 19.05& 19.48&39.09& \textcolor{red}{15.72}& \textcolor{red}{23.67} & \textcolor{red}{51.84}  \\ 
    
     PIT & 2.08& 14.03 & 11.61& 27.15 & 28.86& 27.11 &11.93& \textcolor{red}{15.72}& \textbf{26.31} & 57.58\\
    \selfpt{} & \textbf{1.11}& \textbf{37.25}& \textbf{31.52} & \textbf{50.83}& \textbf{52.62} & \textbf{50.61} &\textbf{44.31}& \textbf{16.45} & 25.67 & \textbf{66.01}\\

    \midrule
        \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-10-Multi (Multi-Domain Scenario)}}\cr
    \midrule
    \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    Open-book w/ test doc & 7.84&48.93&26.63&60.37&71.71&58.54&6.33&-&-&-\\
    Closed-book & 7.84&4.53&2.73&16.19&18.63&16.38&6.33&16.05&24.67 & 53.40\\
    \midrule
   \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    Cont. Pre-training & 3.32&5.86&3.40&18.04&20.59&18.42&14.51&\textbf{17.02}&25.05&53.56\\
    
    Standard Ins.-tuning & 2.73& 8.66 & 5.73& 24.94& 25.64& 25.31 & 34.91& \textcolor{red}{15.60}& 26.26 & \textcolor{red}{52.74} \\ 
    
     % Mixed Training & 1.47 &  16.91& 12.25 & 34.48&35.20 & 34.41 &29.44&\textbf{17.75}&\textbf{28.68} &59.38\\ 
     
     PIT & 1.96& 14.31 & 8.72& 30.26 & 33.97& 30.22 &10.69&\textcolor{red}{15.55} & \textbf{27.02} & 55.12 \\ 
     
      \selfpt{} & \textbf{1.13} & \textbf{22.30}& \textbf{16.51} & \textbf{39.94}& \textbf{41.02} & \textbf{39.89}  & \textbf{50.65}& 16.34 & 25.85 & \textbf{69.29}\\ 
      
       % \selfpt{}$^{++}$ & \textbf{1.09} & \textbf{24.70}& \textbf{17.78} & \textbf{42.95}& \textbf{44.31} & \textbf{42.71} & \textbf{52.61}& \textcolor{red}{14.47} & 25.25 & 66.83\\ 

        \midrule
    \multicolumn{11}{c}{\textbf{Knowledge Acquisition on Wiki-Newpages-2023-(9)10-Film (Cross-Domain Scenario)}}\cr
    \midrule
    % \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/o Knowledge Injection}}}\cr
    % Open-book w/ film doc &8.30&57.38 & 34.45&68.64&78.92&66.31&7.35&-&-&-\\
    Closed-book &8.30&3.35&1.88&11.27&12.97&11.49&7.35&16.05&24.67&53.40\\
    \midrule
   % \multicolumn{8}{l}{\textcolor{lightgray!99}{\textit{w/ Knowledge Injection}}}\cr 
    % Cont. Pre-training &5.52 &3.46&2.30&11.83&14.30&11.98&12.04&\textbf{16.79}& 25.35 & 56.02\\
    % % \hdashline
    % % \noalign{\vskip 0.07cm} % Adds a small vertical space
    % Standard Ins.-tuning &2.83& 5.23 & 3.77& 16.15& 17.45& 16.45& \textbf{51.69}& \textcolor{red}{14.41}& 25.54 & \textcolor{red}{49.80} \\ 

     % Mixed Training &1.47&  11.41& 9.63 & 23.61&24.48 & 23.67 & \textbf{59.99}&\textbf{17.35}&\textbf{27.79} &58.56\\
     
     PIT&1.52& 6.39 & 2.67& 16.97 & 18.92& 17.10 &3.03&\textcolor{red}{13.06} & \textcolor{red}{23.42} & 54.38 \\

     \selfpt{} & \textbf{1.10} & \textbf{22.51}& \textbf{16.44} & \textbf{35.58}& \textbf{36.60} & \textbf{35.43} & 44.92& 16.77& \textbf{26.44} & \textbf{66.34}\\ 
     % \selfpt{}$^{++}$ &\textbf{1.08} & \textbf{44.49}& \textbf{39.82} & \textbf{58.44}& \textbf{60.58} & \textbf{58.00}  & 53.91 & 20.46 & \textbf{32.01} & \textbf{72.48}\\
    \bottomrule  
    \end{tabular}
  \end{threeparttable}
  \caption{Five-shot evaluation results on \llamaa{} for knowledge acquisition and retention in three scenarios: single-domain (top), multi-domain (middle), and cross-domain (bottom). Results that fall below the baseline performance are highlighted in \textcolor{red}{red}.}
  \label{tab:short-bio-domain}
  \vspace{-3.5mm}
\end{table*}

%In the cross-domain scenario, the training data comes from Wiki-Bio, while the testing data is from Wiki-Film.
